Discriminative Nearest Neighbor Few-Shot Intent Detection by Transferring Natural Language Inference

Intent detection is one of the core components of goal-oriented dialog systems, and detecting out-of-scope (OOS) intents is also a practically important skill. Few-shot learning is attracting much attention to mitigate data scarcity, but OOS detection becomes even more challenging. In this paper, we present a simple yet effective approach, discriminative nearest neighbor classification with deep self-attention. Unlike softmax classifiers, we leverage BERT-style pairwise encoding to train a binary classifier that estimates the best matched training example for a user input. We propose to boost the discriminative ability by transferring a natural language inference (NLI) model. Our extensive experiments on a large-scale multi-domain intent detection task show that our method achieves more stable and accurate in-domain and OOS detection accuracy than RoBERTa-based classifiers and embedding-based nearest neighbor approaches. More notably, the NLI transfer enables our 10-shot model to perform competitively with 50-shot or even full-shot classifiers, while we can keep the inference time constant by leveraging a faster embedding retrieval model.

==> misc.tex <==

% \begin{table*}[]
% \centering
% \small
% \resizebox{0.8\linewidth}{!}{
% \begin{tabular}{l|cc|cc|cc|cc}
% \hline
%                      & \multicolumn{2}{c|}{\textbf{In-Domain accuracy}}  & \multicolumn{2}{c|}{\textbf{OOS recall}}          & \multicolumn{2}{c|}{\textbf{OOS precision}}                     & \multicolumn{2}{c}{\textbf{Latency [sec./example]}} \\
% \textbf{Banking}              & \textbf{5-Shot}         & \textbf{10-Shot}        & \textbf{5-Shot}         & \textbf{10-Shot}        & \textbf{5-Shot}                       & \textbf{10-Shot}        & \textbf{5-Shot}  & \textbf{10-Shot}  \\ \hline
% tf-idf               & 59.2 $\pm$ 3.6          & 65.9 $\pm$ 3.8          & 61.0 $\pm$ 2.8          & 51.3 $\pm$ 1.6          & \textbf{97.8 $\pm$ 0.6}               & \textbf{98.2 $\pm$ 0.3} & 0.001                & 0.001                 \\
% sbert-nli            & 78.4 $\pm$ 2.4          & 84.3 $\pm$ 1.2          & 92.1 $\pm$ 2.0          & 91.6 $\pm$ 1.2          & 91.4 $\pm$ 0.8                        & 93.7 $\pm$ 0.5          & 0.017   & 0.017   \\
% nli-Fine-Tune        & 88.6 $\pm$ 1.3          & 91.2 $\pm$ 1.1          & 94.7 $\pm$ 1.0          & 94.8 $\pm$ 1.1          & 97.0 $\pm$ 0.3                        & 97.5 $\pm$ 0.4          & 0.073            & 0.143             \\ 
% Joint-nli (top 20)         & \textbf{88.5 $\pm$ 1.2} & \textbf{91.0 $\pm$ 1.0} & \textbf{95.0 $\pm$ 0.9} & \textbf{95.2 $\pm$ 1.2} & 96.9 $\pm$ 0.4                        & 97.3 $\pm$ 0.4          & 0.039            & 0.039             \\ \hdashline
% classifier           & 79.7 $\pm$ 1.8          & 85.2 $\pm$ 1.3          & 93.3 $\pm$ 2.9          & 93.3 $\pm$ 1.0          & 92.5 $\pm$ 0.9                        & 94.4 $\pm$ 0.5          & 0.028            & 0.028             \\ \hline
% \textbf{All Domains} & \textbf{5-Shot}         & \textbf{10-Shot}        & \textbf{5-Shot}         & \textbf{10-Shot}        & \textbf{5-Shot}                       & \textbf{10-Shot}        & \textbf{5-Shot}  & \textbf{10-Shot}  \\ \hline
% tf-idf               & 35.4 $\pm$ 0.7          & 31.3 $\pm$ 1.1          & 72.2 $\pm$ 2.1          & 83.1 $\pm$ 1.5          & 24.7 $\pm$ 0.4                        & 23.5 $\pm$ 0.4          & 0.001                & 0.002                 \\
% sbert-nli            &                         &                         &                         &                         &                                       &                         &                  &                   \\
% nli-Fine-Tune        & 84.9 $\pm$ 0.8        & 91.6 $\pm$ 0.3        & 90.1 $\pm$ 1.6        & 83.0 $\pm$ 2.0       & \multicolumn{1}{c}{64.7 $\pm$ 2.5} & 81.4 $\pm$ 2.0        & 0.697                 &       1.498            \\ 
% Joint-nli (top 20)            &   84.5 $\pm$ 0.8          &     91.2 $\pm$ 0.2            & 90.6 $\pm$ 1.6            & 85.1 $\pm$ 1.8                        &         63.6 $\pm$ 2.4                      &      78.4 $\pm$ 2.1                   &               0.037   &             0.041      \\ \hdashline
% classifier           & 77.7 $\pm$ 0.6       & 83.2 $\pm$ 0.6        & 91.9 $\pm$ 1.1        & 92.9 $\pm$ 0.8        & \multicolumn{1}{c}{53.9 $\pm$ 0.8} & 58.2 $\pm$ 1.0        & 0.028          & 0.028            \\ \hline
% \end{tabular}}\caption{Testing results on the banking domain and all the domains, where every method is tested on a single gpu.}
% \label{table:latency}
% \end{table*}

